Benchmarking Deep Graph Generative Models for Optimizing New Drug Molecules for COVID-19

Design of new drug compounds with target properties is a key area of research in generative modeling. We present a small drug molecule design pipeline based on graph-generative models and a comparison study of two state-of-the-art graph generative models for designing COVID-19 targeted drug candidates: 1) a variational autoencoder-based approach (VAE) that uses prior knowledge of molecules that have been shown to be effective for earlier coronavirus treatments and 2) a deep Q-learning method (DQN) that generates optimized molecules without any proximity constraints. We evaluate the novelty of the automated molecule generation approaches by validating the candidate molecules with drug-protein binding affinity models. The VAE method produced two novel molecules with similar structures to the antiretroviral protease inhibitor Indinavir that show potential binding affinity for the SARS-CoV-2 protein target 3-chymotrypsin-like protease (3CL-protease).

==> sec_novelty.tex <==
%\section{Ideas for Novelty and Optimization of current RL algorithm}
% % \begin{table*}[!tp]
% \begin{table*}[!h]
% % \centering
% \caption{Comparison of representative approaches in the recent literature. Abbreviations used: FG (functional group).}
% \vspace{-2.5mm}
% \small
% % \resizebox{\linewidth}{!}{
% % \begin{tabular}{l*{4}{c}r}
% \begin{tabular}{| l | p{1.5 cm} | p{1.5cm} | p{1.2 cm} | p{3.0cm} | p{5 cm} |}
% \hline 
% % \toprule[1.5pt]
% \bf Method &\bf Encoding &\bf Action &\bf Reward &\bf Learning Approach &\bf Synthesizability approach \\
% \hline
% GCPN \cite{GCPN} & GCN & Atom or FG & Additive & PPO1 & Inclusion of SAScore  \\\hline
% Mol-DQN \cite{MolDQN} & Morgan  & Atom & Additive  & DQN & SAScore  \\\hline
% JTVAE \cite{JTVAE-multi} & TBD & TBD & TBD & TBD & TBD  \\\hline
% MolGAN (JP) \cite{de2018molgan} & TBD & TBD & TBD & TBD & TBD  \\\hline
% GraphNVP \cite{madhawa2019graphnvp} & TBD & TBD & TBD & TBD & TBD  \\\hline
% GraphAF (JP) \cite{shi2020graphaf} & TBD & TBD & TBD & TBD & TBD  \\\hline
% ChemBO (JP) \cite{korovina2020chembo} & TBD & TBD & TBD & BO on graphs & Bayesian optimization  \\\hline
% Molecule-Chef (GS) \cite{bradshaw2019model} & TBD & TBD & TBD & Graph NN + MT & Reaction prediction (Molecular Transformer) \\\hline
% Molecule-Chef (GS) \cite{gottipati2020learning} & TBD & TBD & TBD & RL & Search synthesizable chemical space \\\hline
% ExaDesign-MolDQN (LW) & Morgan & Atom & Additive & DQN & SAScore (current baseline)  \\\hline
% ExaDesign-MolDQN (LW) & Morgan & Atom & Additive & DQN & Post-process w/ low-shot filter \textbf{(2.2.5)} \\\hline
% ExaDesign-MolDQN (LW) & Morgan & Atom \textbf{(2.2.5)} & Additive & DQN & Inclusion of SAScore  \\\hline
% ExaDesign-MolDQN (LW) & Morgan & Atom & Additive & DQN, better init. \textbf{(2.2.2)} & Inclusion of SAScore  \\\hline
% ExaDesign-TFA (SC) & Morgan & Atom & Additive & DQN + Pretraining  & Inclusion of SAScore  \\\hline
% ExaDesign-TFA (SC) & Morgan & Atom & Additive & DDQN/PPO  & Inclusion of SAScore  \\\hline
% ExaDesign-TFA (SC) & GCN & Atom & Additive & DQN  & Inclusion of SAScore  \\\hline
% ExaDesign-TFA (SC) & best of M/G & best of A/FG & Additive & best of DQN/DDQN/PPO  & Inclusion of SAScore  \\\hline

% ExaDesign (ours) & GCN & Atom or FG & Additive & DQN & Inclusion of SAScore  \\\hline
% ExaDesign (ours) & Morgan & FG? & Additive & DQN, better init. struct & Inclusion of SAScore  \\\hline
% ExaDesign (ours) & TBD & TBD & TBD & TBD & TBD  \\\hline
% ExaDesign (ours) & TBD & TBD & TBD & TBD & TBD  \\\hline
% ExaDesign (ours) & TBD & TBD & TBD & TBD & TBD  \\\hline
% ExaDesign (ours) & TBD & TBD & TBD & TBD & TBD  \\\hline
% ExaDesign (ours) & TBD & TBD & TBD & TBD & Add recent papers  \\\hline
% \end{tabular}
% % }
% \label{tab:related_work}
% \vspace{-3mm}
% \end{table*}

\subsection{Better representation learning}

\begin{enumerate}
    \item Right now we perform Morgan fingerprinting of each molecule.  Check what other state-of-the-art papers do.  Can we use pre-trained embeddings of atoms and functional groups, so that the embeddings are kept close (or far) in vector space based on their relations (participating in a molecule, or reaction)?
    \item Review embedding learning technique used by GCPN paper.
\end{enumerate}

\subsection{Better strategy for Molecule Design}

\begin{enumerate}
    \item \textbf{Dynamic weighting of objectives}  Our current reward assigns equal weight to each objective (pIC50, logP, QED etc.).  Learn how to prioritize the objectives as the molecule is built step-by-step.  See \cite{abels2019dynamic}.
    \item \textbf{Better initiatilization of search (like JTVAE)} Initiate the search from a template structure instead of searching from a single molecule.  Think about how to bring in ``junction tree'' like ideas here.  Learn coarsened representations of a full-fledged molecule, where super-nodes represents functional groups and thus, the coarsened structure becomes a ``template''.  Review ideas from JT-VAE variants and this paper \cite{ying2018hierarchical} for such an approach.  
    \item \textbf{Proximity/template based Reasoning about synthesizability} Currently, we generate a molecule based on specified targets.  Following the literature on graph-based reasoning - we can cast the problem as generate a molecule that satisfies the target properties and show the functional group based template structure to reason about it's synthesizability.  The problem statement in \cite{das2017go} is representative about this body of literature.  
    \item \textbf{Fine-grained decision problem} At each step determine what bond to add, where to add etc.  We talked about this last week.  GCPN uses this approach.
    \item \textbf{Add database similarity to score} Use Learned Similarity (via one-shot GNN approach) to provide a score for if the final molecule and/or intermediate steps are similar to molecules in the database.
\end{enumerate}

\subsection{Better RL approach}

\begin{enumerate}
    \item \textbf{When MLP falls short} The core component in our RL pipeline is the MLP and that can be a limiting factor for learning in a high-dimensional space.  This is not about the speed of convergence, but the the ability for the MLP to effectively map the input molecular representation to accurately estimating values which are again derived from a multi-dimensional vector space (representing multi-objectives).  We have not given much thought to other policies such as PPO (used by GCPN) and actor-critic variants.
\end{enumerate}

